Complexity of Manipulation in Elections with Top-truncated Ballots

In the computational social choice literature, there has been great interest in understanding how computational complexity can act as a barrier against manipulation of elections. Much of this literature, however, makes the assumption that the voters or agents specify a complete preference ordering over the set of candidates. There are many multiagent systems applications, and even real-world elections, where this assumption is not warranted, and this in turn raises the question "How hard is it to manipulate elections if the agents reveal only partial preference orderings?" It is this question we try to address in this paper. In particular, we look at the weighted manipulation problem -- both constructive and destructive manipulation -- when the voters are allowed to specify any top-truncated ordering over the set of candidates. We provide general results for all scoring rules, for elimination versions of all scoring rules, for the plurality with runoff rule, for a family of election systems known as Copeland$^{\alpha}$, and for the maximin protocol. Finally, we also look at the impact on complexity of manipulation when there is uncertainty about the non-manipulators' votes.

==> references.tex <==
\thebibliography{}

\bibitem{bartholdi} Bartholdi III, John J., Craig A. Tovey, and Michael A. Trick. ``The computational difficulty of manipulating an election." Social Choice and Welfare 6.3 (1989): 227-241.

\bibitem{baumeister} Baumeister, Dorothea, et al. ``Campaigns for lazy voters: Truncated ballots." Proceedings of the 11th International Conference on Autonomous Agents and Multiagent Systems-Volume 
2. International Foundation for Autonomous Agents and Multiagent Systems, 2012.

\bibitem{coleman} Coleman, Tom, and Vanessa Teague. ``On the complexity of manipulating elections.'' Proceedings of the thirteenth Australasian symposium on Theory of computing-Volume 65. Australian 
Computer Society, Inc., 2007.

\bibitem{conitzer} Conitzer, Vincent, Tuomas Sandholm, and Jérôme Lang. ``When are elections with few candidates hard to manipulate?." Journal of the ACM (JACM) 54.3 (2007): 14.

\bibitem{jessica} Davies, Jessica, Nina Narodytska, and Toby Walsh. ``Eliminating the weakest link: Making manipulation intractable?.'' arXiv preprint arXiv:1204.3918 (2012).

\bibitem{falis} Faliszewski, Piotr, Edith Hemaspaandra, and Henning Schnoor. ``Copeland voting: Ties matter." Proceedings of the 7th international joint conference on Autonomous agents and multiagent 
systems-Volume 2. International Foundation for Autonomous Agents and Multiagent Systems, 2008.

\bibitem{falis2} Faliszewski, Piotr, and Ariel D. Procaccia. ``AI's war on manipulation: Are we winning?." AI Magazine 31.4 (2010): 53-64.

\bibitem{falis3} Faliszewski, Piotr, Edith Hemaspaandra, and Lane A. Hemaspaandra. ``Using complexity to protect elections." Communications of the ACM 53.11 (2010): 74-82.

\bibitem{friedgut} Friedgut, Ehud, Gil Kalai, and Noam Nisan. ``Elections can be manipulated often.'' Hebrew University, Center for the study of Rationality, 2008.

\bibitem{nina} Narodytska, Nina, and Toby Walsh. ``The computational impact of partial votes on strategic voting." Proceedings of the 21st European Conference on Artificial Intelligence (ECAI 2014).

\bibitem{procaccia} Procaccia, Ariel D., Jeffrey S. Rosenschein, and Gal A. Kaminka. ``On the robustness of preference aggregation in noisy environments." Proceedings of the 6th international joint 
conference on Autonomous agents and multiagent systems. ACM, 2007.

\bibitem{procaccia2} Procaccia, Ariel D., and Jeffrey S. Rosenschein. ``Junta distributions and the average-case complexity of manipulating elections." Proceedings of the fifth international joint 
conference on Autonomous agents and multiagent systems. ACM, 2006.

\bibitem{procaccia3} Procaccia, Ariel D., and Jeffrey S. Rosenschein. ``Average-case tractability of manipulation in voting via the fraction of manipulators." AAMAS. 2007.

\bibitem{xia} Xia, Lirong, and Vincent Conitzer. ``Determining possible and necessary winners under common voting rules given partial orders." Journal of Artificial Intelligence Research 41.2 (2011): 
25-67.


